Performance of the LHCb RICH detector at the LHC

The LHCb experiment has been taking data at the Large Hadron Collider (LHC) at CERN since the end of 2009. One of its key detector components is the Ring-Imaging Cherenkov (RICH) system. This provides charged particle identification over a wide momentum range, from 2-100 GeV/c. The operation and control software, and online monitoring of the RICH system are described. The particle identification performance is presented, as measured using data from the LHC. Excellent separation of hadronic particle types (pion, kaon and proton) is achieved.

==> aliases.tex <==
% $Id: aliases.tex 28 2010-10-05 15:19:02Z tskwarni $
% ===============================================================================
% Purpose: use of predefined symbols in the standard template
% Author: Tomasz Skwarnicki
% Created on: 2010-09-24
% ===============================================================================

\section{Aliases}
\label{sec:Aliases}

Some collaborations standardize typesetting of their symbols, particle, units etc.\ 
by defining standard macros (aliases) for them. 
While uniform typesetting of all LHCb documents would be good, 
this would come at the price of having to get used to typing the alias names. 

At this time we do not impose the use of such aliases. 
However, a proposal and the necessary files are included in the appendix.
People who like the idea should feel free to use them.
If you were going to use your own aliases you are strongly encouraged to use the standard 
alias template instead!


==> figures.tex <==
% $Id: figures.tex 28 2010-10-05 15:19:02Z tskwarni $
% ===============================================================================
% Purpose: including figures in the standard template
% Author: Tomasz Skwarnicki
% Created on: 2010-09-24
% ===============================================================================

\section{Figures}
\label{sec:Figures}

At this point we are not imposing a standard package for including figures.
Packages usually come with restrictions on file types which can be included. 
Which figure types are included affects also how output file is obtained from the source tex files.

Below we show an example how to include eps or pdf figure with 
\texttt{\textbackslash includegraphics} command (eps figures will not work with \texttt{pdflatex}).

\begin{figure}[htbp]
  \begin{center}
  \ifthenelse{\boolean{pdflatex}}{
    \includegraphics*[width=0.7\textwidth]{figs/example_plot.pdf}
   }{
    \includegraphics*[width=0.7\textwidth]{figs/example_plot.eps}
   } 
  \end{center}
  \caption{\small The unitarity triangle.}
  \label{fig:triangle}
\end{figure}


